Infinite Determinantal Measures and The Ergodic Decomposition of Infinite Pickrell Measures I. Construction of infinite determinantal measures

This paper is the first in a series of three. The main result, Theorem 1.11, gives an explicit description of the ergodic decomposition for infinite Pickrell measures on spaces of infinite complex matrices. The main construction is that of sigma-finite analogues of determinantal measures on spaces of configurations. An example is the infinite Bessel point process, the scaling limit of sigma-finite analogues of Jacobi orthogonal polynomial ensembles. The statement of Theorem 1.11 is that the infinite Bessel point process (subject to an appropriate change of variables) is precisely the ergodic decomposition measure for infinite Pickrell measures.

==> extref-arxiv.tex <==
% File for inter-part referencing
%------ Macros

\makeatletter

\newcommand{\newlonglabel}[3]{
\def\@@foo{#2}%
\ifx\thispartnum\@@foo\relax
\@bsphack\protected@write\@auxout{}{\string\checklonglabel{#1}{#3}}\@esphack
\else
\@bsphack\protected@write\@auxout{}{\string\newlabel{#1}{{#2.#3}{--}}}\@esphack
\fi
}
\let\checklonglabel\@gobbletwo

\AtEndDocument{\def\checklonglabel#1#2{{\@ifundefined{r@#1}%
{\GenericWarning{}{Longlabel `#1' of this part has label of the same name undefined}}%
{\edef\@@foox{\expandafter\expandafter\expandafter\@firstoftwo\csname r@#1\endcsname}\def\@@fooy{#2}%
\ifx\@@foox\@@fooy\relax\else
\GenericWarning{}{Longlabel `#1' of this part does not coincide with the label of the same name}%
\fi}}}}

\let\longref=\ref
\makeatother


%------ Part I

\newlonglabel{asympt-R-bessel}{I}{1.3}
\newlonglabel{bs-sing}{I}{1.4}
\newlonglabel{singul}{I}{1.9}
\newlonglabel{mainthm-fin}{I}{1.10}
\newlonglabel{mainthm}{I}{1.11}
\newlonglabel{main-lemma}{I}{1.14}
\newlonglabel{expbetaint}{I}{1.15}
\newlonglabel{weak-pick}{I}{1.16}
\newlonglabel{rad-jac}{I}{1.17}
\newlonglabel{det-CDJ}{I}{5}
\newlonglabel{expaa}{I}{8}
\newlonglabel{pisb}{I}{9}
\newlonglabel{rinftymu}{I}{14}
\newlonglabel{rad-u-coord}{I}{17}

\newlonglabel{infdet-he}{I}{2.11}
\newlonglabel{mult-he1}{I}{2.14}
\newlonglabel{closedsubsp}{I}{2.18}
\newlonglabel{fin-rank-mult}{I}{2.19}
\newlonglabel{lin-ind}{I}{2.21}
\newlonglabel{lve}{I}{3}
\newlonglabel{def-Pi-g}{I}{21}

\newlonglabel{tilde-kernel-kns-js}{I}{A.3}
\newlonglabel{CDJ}{I}{34}

\newlonglabel{fin-distr-unique}{I}{B.1}
\newlonglabel{pr1-bis}{I}{B.3}

\newlonglabel{inf-prod-s}{I}{40}

%------ Part II

\newlonglabel{conv-induced}{II}{2.3}
\newlonglabel{conv-inf-det}{II}{2.6}
\newlonglabel{conv-unif-finrank}{II}{3.13}

%------ Part III

% None

\endinput

